OEKG: The Open Event Knowledge Graph

Accessing and understanding contemporary and historical events of global impact such as the US elections and the Olympic Games is a major prerequisite for cross-lingual event analytics that investigate event causes, perception and consequences across country borders. In this paper, we present the Open Event Knowledge Graph (OEKG), a multilingual, event-centric, temporal knowledge graph composed of seven different data sets from multiple application domains, including question answering, entity recommendation and named entity recognition. These data sets are all integrated through an easy-to-use and robust pipeline and by linking to the event-centric knowledge graph EventKG. We describe their common schema and demonstrate the use of the OEKG at the example of three use cases: type-specific image retrieval, hybrid question answering over knowledge graphs and news articles, as well as language-specific event recommendation. The OEKG and its query endpoint are publicly available.

==> example_queries/uner_mlm.tex <==

SELECT DISTINCT ?image
WHERE
{
?earthquake rdf:type uner:Earthquake .
?earthquake sem:hasPlace ?location .
?location so:image ?image .
}

==> example_queries/vquanda_news.tex <==

SELECT ?questionText ?answerText ?headline ?mainEnt ?answerEntity
WHERE
{
?question so:suggestedAnswer ?answer;
 so:mainEntity ?mainEnt ;
 so:text ?questionText .
?answer so:mentions ?answerEntity1 ;
         so:text ?answerText .

?answerEntity rdf:type sem:Event .
FILTER(?mainEnt != ?answerEntity) .
  
?article rdf:type so:Article .
?article so:mentions ?answerEntity , ?mainEnt ;
 so:headline ?headline .
} LIMIT 1

==> image_links.tex <==
https://www.openstreetmap.org/copyright/en

https://commons.wikimedia.org/wiki/File:Hanover_banner_1.jpg
https://commons.wikimedia.org/wiki/File:Neues_Rathaus_Hannover_M%C3%A4rz_2010.jpg

https://commons.wikimedia.org/wiki/File:Messina_harbour_-_aerial_view.jpg
https://commons.wikimedia.org/wiki/File:Castello_esterno.jpg
https://commons.wikimedia.org/wiki/File:Guaranda_(284885979).jpg
